Many universality classes in an interface model restricted to non-negative heights

We present a simple one dimensional stochastic model with three control parameters and a surprisingly rich zoo of phase transitions. At each (discrete) site $x$ and time $t$, an integer $n(x,t)$ satisfies a linear interface equation with added random noise. Depending on the control parameters, this noise may or may not satisfy the detailed balance condition, so that the growing interfaces are in the Edwards-Wilkinson (EW) or in the Kardar-Parisi-Zhang (KPZ) universality class. In addition, there is also a constraint $n(x,t) \geq 0$. Points $x$ where $n>0$ on one side and $n=0$ on the other are called ``fronts". These fronts can be ``pushed" or ``pulled", depending on the control parameters. For pulled fronts, the lateral spreading is in the directed percolation (DP) universality class, while it is of a novel type for pushed fronts, with yet another novel behavior in between. In the DP case, the activity at each active site can in general be arbitrarily large, in contrast to previous realizations of DP. Finally, we find two different types of transitions when the interface detaches from the line $n=0$ (with $\langle n(x,t)\rangle \to$ const on one side, and $\to \infty$ on the other), again with new universality classes. We also discuss a mapping of this model to the avalanche propagation in a directed Oslo rice pile model in specially prepared backgrounds.

==> Empty_Document <==
PROBLEMS WITH MANUSCRIPT:

The following problems were noted in your manuscript.

* It appears that some of your reference citations are not in order.
  Please ensure that the initial citations appear in consecutive
  numerical order.

In reviewing the figures of your paper, we note that the following
changes would be needed in order for your figures to conform to the
style of the Physical Review.  Please check all figures for the
following problems and make appropriate changes in the text of the
paper itself wherever needed for consistency.

* Please ensure that your figures, captions, and text references to
  these figures are appropriate for both color and grayscale. Many
  standard colors have similar grayscale values and therefore may be
  indistinguishable in any printout. For example, reference to a "blue
  line" and a "red line" in a figure is insufficient, as these labels
  are meaningless for the grayscale version. Mention shading or
  location as an additional description in the caption ["the green
  (light gray) line," "the green (upper) line"], or use different
  styles of curves ("dotted blue line," "dashed red line") or data
  point symbols ("blue circle," "red square") in the figures.

----------------------------------------------------------------------
Report of the First Referee -- EZ12124/Grassberger
----------------------------------------------------------------------

This is an interesting paper produced by fertile collaboration amongst
seasoned professionals.

They introduce a rich, but simply defined model capturing a wealth of
nonequilibrium statistical mechanical phenomena in a complicated phase
diagram, including Kardar-Parisi-Zhang and Edwards-Wilkinson scaling,
but also variants of directed percolation, as well as pushed, pulled &
pinned fronts.

There's a lot going on here and the analysis is hard-core numerical in
the evidence it presents, but the ties to various past [Reggeon Field
Theory] and present [Oslo Rice Model, epidemiology of helminth
infections, etc...] areas of interest to the field, along w/ its key
improvement upon DP [i.e. that is, the authors build in the
possibility of sites being active to varying degrees, not simply
on/off...] clearly will make the manuscript of great interest of the
readership of PRE.

For this reason, as well as the extraordinary track record of the
authors and the serendipity of this collaboration, it's a safe bet
that the manuscript will trigger future valuable work.

----------------------------------------------------------------------
Report of the Second Referee -- EZ12124/Grassberger
----------------------------------------------------------------------

The paper introduces a one-dimensional cellular automaton model that
mimics the height of a stochastic growth model in 1D. The interface
has a barrier at h=0 to/from which it can become attached/detached.
The model has three free parameters producing a complicated map of
phases. Almost magically these phases seem to include many of the
prototypical universal dynamics out-of-equilibrium. KPZ, DP, epidemic
spreading, SOC rice-piles, etc The numerical results that give support
to this associations are not always optimal, some are even weak, due
to crossover effects or/and extremely long transients.

I have several questions comments:

1) It seems that the "peculiar" periodic dependence of the velocity
with the tilt is on the basis of the explosion of the number of
dynamical phases that are found. However, this periodic velocity has
never been reported in any real or theoretical model as far as I know
(apart form an unpublished manuscript by the same author and on the
same model). I wonder what is the physical meaning or relevance of
this periodic v. I mean, the physics behind the tilt-dependence of v
in the usual situation is clear, the interface velocity changes (if
nonlinearites are present) when the whole system is tilted. Actually,
the precise form of the nonlinear terms can be directly inferred from
v(a). In KPZ one finds v(a) ~ a^2 because of the (\nabla h)^2 term. In
what type of system would the velocity depend periodically on a? Would
this imply that the nonlinear term is some periodic function of \nabla
h?

2) On page 5, just before subsection 3. Directed percolation the paper
says: "which would be analogous to using improved Hamiltionians ..".
Please explain what do you mean by improved Hamiltonians and how that
could help to avoid crossover effects. As far as I know there have
been a number of (often hot) discussions in many classical
non-equilibrium models about if the model is in this or that
universality class. Never heard of the above mentioned method to tell
apart two universality classes, at least out-of-equilibrium larger
systems and longer simulations use to be the only general method to
deal with these type of questions.

Minor points and typos:

- Abstract says two control parameters, in Conclusions section it says
three.

- where "a" stands for barrier, should be "b"

- "close by an inflection point, of because" --> or because

- Page 3 last paragraph, "because" at paragraph beginning.

- Section IV.B.4 just below Fig 9, "Finally, panel (c) shows ..." -->
"Finally, panel (d) shows ..."

- Same typo just before Eq(10)

- Page 11, just after Eq(15), "Notice that the mapping Eq.(16)" -->
Eq(15)

- I think the same typo applies in the text just after Eq(16),
"Using..." and at the end of the paragraph "In the latter case ..."

- Axis label should be enlarged in all plots, at double column format
lettering is very small as it is.

- I would recommend to change all axis numbers to scientific notation,
avoid 100 and 1000000 and use 10^2 and 10^6 everywhere as it is some
axes are messy.

I recommend publication after the authors have considered my comments
above.

